Empowering Image Recovery_ A Multi-Attention Approach

We propose Diverse Restormer (DART), a novel image restoration method that effectively integrates information from various sources (long sequences, local and global regions, feature dimensions, and positional dimensions) to address restoration challenges. While Transformer models have demonstrated excellent performance in image restoration due to their self-attention mechanism, they face limitations in complex scenarios. Leveraging recent advancements in Transformers and various attention mechanisms, our method utilizes customized attention mechanisms to enhance overall performance. DART, our novel network architecture, employs windowed attention to mimic the selective focusing mechanism of human eyes. By dynamically adjusting receptive fields, it optimally captures the fundamental features crucial for image resolution reconstruction. Efficiency and performance balance are achieved through the LongIR attention mechanism for long sequence image restoration. Integration of attention mechanisms across feature and positional dimensions further enhances the recovery of fine details. Evaluation across five restoration tasks consistently positions DART at the forefront. Upon acceptance, we commit to providing publicly accessible code and models to ensure reproducibility and facilitate further research.

==> DART/figures/visual_dn.tex <==
\begin{figure*}[!tb]
\begin{center}
\scriptsize
% \scalebox{0.97}{
\begin{tabular}[b]{c@{ } c@{ } c@{ } c@{ }}
\hspace{-2mm}  
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_003_gt.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_003_noisy.png} & 
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_003_sgn.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_003_drunet.png} \\
    Ground-truth & Noisy & SGN~\cite{gu2019self} & DRUNet~\cite{zhang2021plug}  \\
\hspace{-2mm}  
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_003_ipt.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_003_swinir.png} & 
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_003_restormer.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_003_grl.png} \\ 
    IPT~\cite{chen2021pre} & SwinIR~\cite{liang2021swinir} & Restormer~\cite{zamir2022restormer} & GRL  \\ \\
\hspace{-2mm}  
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_004_gt.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_004_noisy.png} & 
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_004_sgn.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_004_drunet.png} \\
    Ground-truth & Noisy & SGN~\cite{gu2019self} & DRUNet~\cite{zhang2021plug}  \\
\hspace{-2mm}  
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_004_ipt.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_004_swinir.png} & 
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_004_restormer.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_004_grl.png} \\ 
    IPT~\cite{chen2021pre} & SwinIR~\cite{liang2021swinir} & Restormer~\cite{zamir2022restormer} & GRL  \\ \\
% \hspace{-2mm}  
%     \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_005_gt.png} &
%     \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_005_noisy.png} & 
%     \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_005_sgn.png} &
%     \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_005_drunet.png} \\
    % Ground-truth & Noisy & SGN~\cite{gu2019self} & DRUNet~\cite{zhang2021plug}  \\
% \hspace{-2mm}  
%     \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_005_ipt.png} &
%     \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_005_swinir.png} & 
%     \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_005_restormer.png} &
%     \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_005_grl.png} \\ 
    % IPT~\cite{chen2021pre} & SwinIR~\cite{liang2021swinir} & Restormer~\cite{zamir2022restormer} & GRL  \\ \\
\hspace{-2mm}  
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_012_gt.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_012_noisy.png} & 
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_012_sgn.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_012_drunet.png} \\
    Ground-truth & Noisy & SGN~\cite{gu2019self} & DRUNet~\cite{zhang2021plug}  \\
\hspace{-2mm}  
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_012_ipt.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_012_swinir.png} & 
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_012_restormer.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_012_grl.png} \\ 
    IPT~\cite{chen2021pre} & SwinIR~\cite{liang2021swinir} & Restormer~\cite{zamir2022restormer} & GRL  \\ \\
\end{tabular}
% }
\end{center}
% \vspace{-4mm}
\caption{Visual results for color image denoising. The noise level is 50. Compared with the other methods, the proposed method could restore more details in the input image while removing severe noise from the input images.}
% Instead, the combination of the horizontal and vertical stripes and their shifted version could be well suited to the anisotropic features. Conducting self-attention could further reduce the computational complexity and maintain the long-range modelling capacity.}
\label{fig:supp_visual_dn}
% \vspace{-6mm}
\end{figure*}


==> DART/figures/visual_dpdd.tex <==
\begin{figure*}[!tb]
\begin{center}
\scriptsize
% \scalebox{0.97}{
\begin{tabular}[b]{c@{ } c@{ } c@{ } c@{ }}
\hspace{-2mm}  
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A2316_lq.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A2316_uformer.png} & 
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A2316_restormer.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A2316_grl.png} \\ \\
\hspace{-2mm}  
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A0995_lq.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A0995_uformer.png} & 
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A0995_restormer.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A0995_grl.png} \\ \\
\hspace{-2mm}  
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A1652_lq.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A1652_uformer.png} & 
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A1652_restormer.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A1652_grl.png} \\ \\
\hspace{-2mm}  
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A2002_lq.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A2002_uformer.png} & 
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A2002_restormer.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A2002_grl.png} \\ \\

    Blurred & Uformer~\cite{wang2022uformer} & Restormer~\cite{zamir2022restormer} & GRL  \\
\end{tabular}
% }
\end{center}
% \vspace{-4mm}
\caption{Visual results for dual-pixel defocus deblurring. Compared with other methods, the proposed method could remove more blurriness from the input image.}
% Instead, the combination of the horizontal and vertical stripes and their shifted version could be well suited to the anisotropic features. Conducting self-attention could further reduce the computational complexity and maintain the long-range modelling capacity.}
\label{fig:supp_visual_dpdd}
% \vspace{-6mm}
\end{figure*}


==> DART/figures/visual_motion_db.tex <==
\begin{figure*}[!tb]
\begin{center}
\scriptsize
% \scalebox{0.97}{
\begin{tabular}[b]{c@{ } c@{ } c@{ } c@{ } c@{ }}
\hspace{-2mm}  
    \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0410_11_00_00000069_lq.png} &
    \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0410_11_00_00000069_mprnet.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0410_11_00_00000069_uformer.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0410_11_00_00000069_restormer.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0410_11_00_00000069_grl.png}  \\ \\
\hspace{-2mm}  
    \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0854_11_00_00000089_lq.png} &
    \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0854_11_00_00000089_mprnet.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0854_11_00_00000089_uformer.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0854_11_00_00000089_restormer.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0854_11_00_00000089_grl.png}  \\ \\
\hspace{-2mm}  
    \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0862_11_00_00000043_lq.png} &
    \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0862_11_00_00000043_mprnet.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0862_11_00_00000043_uformer.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0862_11_00_00000043_restormer.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0862_11_00_00000043_grl.png}  \\ \\
\hspace{-2mm}  
    \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0881_11_01_00000012_lq.png} &
    \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0881_11_01_00000012_mprnet.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0881_11_01_00000012_uformer.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0881_11_01_00000012_restormer.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0881_11_01_00000012_grl.png}  \\ \\
    Blurred & MPRNet~\cite{zamir2021multi} & Uformer~\cite{wang2022uformer} & Restormer~\cite{zamir2022restormer} & GRL (Ours) \\
\end{tabular}
% }
\end{center}
% \vspace{-4mm}
\caption{Visual results for single image motion deblurring. The proposed method GRL could recover sharper details compared with the other methods.}
% Instead, the combination of the horizontal and vertical stripes and their shifted version could be well suited to the anisotropic features. Conducting self-attention could further reduce the computational complexity and maintain the long-range modelling capacity.}
\label{fig:supp_visual_motion_db}
% \vspace{-6mm}
\end{figure*}

==> DART/figures/visual_sr.tex <==
\begin{figure*}[!tb]
\begin{center}
\scriptsize
% \scalebox{0.97}{
\begin{tabular}[b]{c@{ } c@{ } c@{ }}
% \hspace{-2mm}  
%     \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_003_gt.png} &
%     \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_003_lr.png} & 
%     \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_003_ipt.png} \\
%     Ground-truth & LR & IPT~\cite{chen2021pre}  \\
% \hspace{-2mm}  
%     \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_003_swinir.png} &
%     \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_003_edt.png} &
%     \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_003_grl.png} \\ 
    % SwinIR~\cite{liang2021swinir} & EDT~\cite{li2021efficient} & GRL  \\ \\
\hspace{-2mm}  
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_019_gt.png} &
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_019_lr.png} & 
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_019_ipt.png} \\
    Ground-truth & LR & IPT~\cite{chen2021pre}  \\
\hspace{-2mm}  
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_019_swinir.png} &
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_019_edt.png} &
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_019_grl.png} \\ 
    SwinIR~\cite{liang2021swinir} & EDT~\cite{li2021efficient} & GRL  \\ \\
\hspace{-2mm}  
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_020_gt.png} &
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_020_lr.png} & 
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_020_ipt.png} \\
    Ground-truth & LR & IPT~\cite{chen2021pre}  \\
\hspace{-2mm}  
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_020_swinir.png} &
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_020_edt.png} &
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_020_grl.png} \\ 
    SwinIR~\cite{liang2021swinir} & EDT~\cite{li2021efficient} & GRL  \\ \\
\hspace{-2mm}  
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_024_gt.png} &
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_024_lr.png} & 
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_024_ipt.png} \\
    Ground-truth & LR & IPT~\cite{chen2021pre}  \\
\hspace{-2mm}  
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_024_swinir.png} &
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_024_edt.png} &
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_024_grl.png} \\ 
    SwinIR~\cite{liang2021swinir} & EDT~\cite{li2021efficient} & GRL  \\ \\

\end{tabular}
% }
\end{center}
\vspace{-4mm}
\caption{Visual results for classical image SR. The upscaling factor is $\times 4$. Compared with other methods, the proposed method could recover more details such as lines and edges in the input LR image.}
% Instead, the combination of the horizontal and vertical stripes and their shifted version could be well suited to the anisotropic features. Conducting self-attention could further reduce the computational complexity and maintain the long-range modelling capacity.}
\label{fig:supp_visual_sr}
% \vspace{-6mm}
\end{figure*}
